Algorithms for Optimal Topology Design, Placement, Sizing and Operation of Distributed Energy Resources in Resilient Off-grid Microgrids

Power distribution in remote communities often depends on off-grid microgrids. In order to address the reliability challenges for these microgrids, we develop a mathematical model for topology design, capacity planning, and operation of distributed energy resources in microgrids that includes N-1 security analysis. Due to the prohibitive size of the optimization problem, we develop a rolling-horizon algorithm that is combined with scenario-based decomposition to efficiently solve the model. We demonstrate the efficiency of our algorithm on an adapted IEEE test network and a real network from an Alaskan microgrid. We also compare our model's required solution time with commercial solvers and recently developed decomposition algorithms to solve similar problems.

==> Data/12-ITGHC-IC96.tex <==
Design_Horizon	IT_IC
1	205000
2	205000
3	205000
4	205000
5	205000
6	205000
7	205000
8	205000
9	205000
10	205000
11	205000
12	205000
13	205000
14	205000
15	205000
16	205000
17	205000
18	205000
19	205000
20	205000
21	205000
22	205000
23	205000
24	205000
25	205000
26	205000
27	205000
28	205000
29	205000
30	205000
31	205000
32	205000
33	205000
34	205000
35	205000
36	205000
37	205000
38	205000
39	205000
40	205000
41	205000
42	205000
43	205000
44	205000
45	205000
46	205000
47	205000
48	205000
49	205000
50	205000
51	205000
52	205000
53	205000
54	205000
55	205000
56	205000
57	205000
58	205000
59	205000
60	205000
61	205000
62	205000
63	205000
64	205000
65	205000
66	205000
67	205000
68	205000
69	205000
70	205000
71	205000
72	205000
73	205000
74	205000
75	205000
76	205000
77	205000
78	205000
79	205000
80	205000
81	205000
82	205000
83	205000
84	205000
85	205000
86	205000
87	205000
88	205000
89	205000
90	205000
91	205000
92	205000
93	205000
94	205000
95	205000
96	205000


==> Data/12-ITGHC-OC96.tex <==
Design_Horizon	IT_OC
1	1531.675438
2	3015.885473
3	6389.413729
4	9021.55001
5	12853.49383
6	14207.4343
7	16456.20599
8	17968.98194
9	19030.76686
10	19840.49082
11	20892.56979
12	21365.67535
13	21809.34182
14	23331.66382
15	25319.60925
16	27568.18445
17	29045.6794
18	29460.2586
19	30247.6841
20	31158.40811
21	31629.69636
22	32053.07147
23	32488.86826
24	32854.48978
25	33220.39253
26	33600.31649
27	33988.05817
28	34365.41632
29	34743.2912
30	35561.30773
31	36102.95584
32	36705.56459
33	37247.65236
34	37725.26394
35	38323.51094
36	39191.70107
37	40270.31471
38	41098.90996
39	43099.54433
40	45271.9612
41	48340.63285
42	52818.35074
43	56974.40379
44	61100.21331
45	62477.56303
46	63893.86047
47	64877.16478
48	65591.36878
49	66268.69508
50	67303.54158
51	68226.7811
52	69474.3323
53	70301.51874
54	70779.12471
55	71412.62891
56	71996.35595
57	72569.85426
58	74015.2309
59	75623.00045
60	76646.05902
61	77365.46514
62	78110.76919
63	79124.99973
64	80034.97501
65	81782.70845
66	83297.4921
67	85988.31246
68	88831.03717
69	91001.40098
70	93803.10826
71	95584.41937
72	97526.46152
73	100373.2082
74	105407.0881
75	110380.4162
76	113978.3706
77	117420.838
78	120777.1405
79	124043.8559
80	125861.5033
81	128523.6616
82	129893.0785
83	133059.4839
84	135761.535
85	137232.7274
86	138777.6703
87	139808.9055
88	140888.341
89	142519.034
90	144244.8437
91	145373.3065
92	146991.8691
93	148372.9459
94	149812.9683
95	151205.2153
96	152430.6505


==> Data/12-ITGHC-TC96.tex <==
Design_Horizon	IT_TC
1	206531.6754
2	208015.8855
3	211389.4137
4	214021.55
5	217853.4938
6	219207.4343
7	221456.206
8	222968.9819
9	224030.7669
10	224840.4908
11	225892.5698
12	226365.6754
13	226809.3418
14	228331.6638
15	230319.6093
16	232568.1844
17	234045.6794
18	234460.2586
19	235247.6841
20	236158.4081
21	236629.6964
22	237053.0715
23	237488.8683
24	237854.4898
25	238220.3925
26	238600.3165
27	238988.0582
28	239365.4163
29	239743.2912
30	240561.3077
31	241102.9558
32	241705.5646
33	242247.6524
34	242725.2639
35	243323.5109
36	244191.7011
37	245270.3147
38	246098.91
39	248099.5443
40	250271.9612
41	253340.6328
42	257818.3507
43	261974.4038
44	266100.2133
45	267477.563
46	268893.8605
47	269877.1648
48	270591.3688
49	271268.6951
50	272303.5416
51	273226.7811
52	274474.3323
53	275301.5187
54	275779.1247
55	276412.6289
56	276996.3559
57	277569.8543
58	279015.2309
59	280623.0005
60	281646.059
61	282365.4651
62	283110.7692
63	284124.9997
64	285034.975
65	286782.7084
66	288297.4921
67	290988.3125
68	293831.0372
69	296001.401
70	298803.1083
71	300584.4194
72	302526.4615
73	305373.2082
74	310407.0881
75	315380.4162
76	318978.3706
77	322420.838
78	325777.1405
79	329043.8559
80	330861.5033
81	333523.6616
82	334893.0785
83	338059.4839
84	340761.535
85	342232.7274
86	343777.6703
87	344808.9055
88	345888.341
89	347519.034
90	349244.8437
91	350373.3065
92	351991.8691
93	353372.9459
94	354812.9683
95	356205.2153
96	357430.6505


==> Data/13-ITNLGHC-IC96.tex <==
Design_Horizon	ITNLHC_IC
1	602735.45
2	602735.45
3	602735.45
4	602735.45
5	602735.45
6	602735.45
7	602735.45
8	602735.45
9	602735.45
10	602735.45
11	602735.45
12	602735.45
13	602735.45
14	602735.45
15	602735.45
16	602735.45
17	602735.45
18	602735.45
19	602735.45
20	602735.45
21	602735.45
22	602735.45
23	602735.45
24	602735.45
25	602735.45
26	602735.45
27	602735.45
28	602735.45
29	602735.45
30	602735.45
31	602735.45
32	602735.45
33	602735.45
34	602735.45
35	602735.45
36	602735.45
37	602735.45
38	602735.45
39	602735.45
40	602735.45
41	602735.45
42	602735.45
43	602735.45
44	602735.45
45	602735.45
46	602735.45
47	602735.45
48	602735.45
49	602735.45
50	602735.45
51	602735.45
52	602735.45
53	602735.45
54	602735.45
55	602735.45
56	602735.45
57	602735.45
58	602735.45
59	602735.45
60	602735.45
61	602735.45
62	602735.45
63	602735.45
64	602735.45
65	602735.45
66	602735.45
67	602735.45
68	602735.45
69	602735.45
70	602735.45
71	602735.45
72	602735.45
73	602735.45
74	602735.45
75	602735.45
76	602735.45
77	602735.45
78	602735.45
79	602735.45
80	602735.45
81	602735.45
82	602735.45
83	602735.45
84	602735.45
85	602735.45
86	602735.45
87	602735.45
88	602735.45
89	602735.45
90	602735.45
91	602735.45
92	602735.45
93	602735.45
94	602735.45
95	602735.45
96	602735.45


==> Data/13-ITNLGHC-OC96.tex <==
Design_Horizon	ITNLHC_OC
1	622.69721
2	1228.963242
3	2530.412721
4	3633.281376
5	5105.759239
6	5670.422279
7	6592.605902
8	7208.164786
9	7652.920598
10	7980.839726
11	8420.736226
12	8631.579971
13	8835.552068
14	9453.305591
15	10215.86449
16	11071.10521
17	11674.20798
18	11873.28188
19	12192.22448
20	12564.97638
21	12779.21061
22	12978.87155
23	13181.17445
24	13370.87911
25	13560.58619
26	13752.37184
27	13945.42699
28	14136.82349
29	14328.30317
30	14659.82773
31	14889.30898
32	15138.03516
33	15367.64871
34	15579.60776
35	15826.87964
36	16180.6953
37	16631.06153
38	16965.36573
39	17724.27565
40	18543.1421
41	19689.44792
42	21358.84888
43	22932.74341
44	24494.39378
45	25063.84285
46	25644.29921
47	26051.80308
48	26342.9111
49	26620.31079
50	27051.83951
51	27430.11517
52	27963.94781
53	28299.28183
54	28511.34613
55	28771.53532
56	29015.98385
57	29256.32021
58	29843.98195
59	30479.17662
60	30903.89149
61	31194.93656
62	31496.16214
63	31917.23201
64	32289.20996
65	32967.53326
66	33576.35143
67	34580.91764
68	35641.55065
69	36460.33068
70	37505.7523
71	38193.96674
72	38933.6215
73	39994.24363
74	41855.59134
75	43697.16841
76	45044.88335
77	46332.02962
78	47585.56045
79	48804.64826
80	49504.03354
81	50496.17134
82	51063.32985
83	52244.01233
84	53250.78093
85	53846.82918
86	54464.21838
87	54894.02024
88	55347.78228
89	55990.48714
90	56661.77467
91	57140.34527
92	57779.54861
93	58350.13118
94	58937.36881
95	59511.09454
96	60039.00493


==> Data/13-ITNLGHC-TC96.tex <==
Design_Horizon	ITNLHC_TC
1	603358.1472
2	603964.4132
3	605265.8627
4	606368.7314
5	607841.2092
6	608405.8723
7	609328.0559
8	609943.6148
9	610388.3706
10	610716.2897
11	611156.1862
12	611367.03
13	611571.0021
14	612188.7556
15	612951.3145
16	613806.5552
17	614409.658
18	614608.7319
19	614927.6745
20	615300.4264
21	615514.6606
22	615714.3215
23	615916.6245
24	616106.3291
25	616296.0362
26	616487.8218
27	616680.877
28	616872.2735
29	617063.7532
30	617395.2777
31	617624.759
32	617873.4852
33	618103.0987
34	618315.0578
35	618562.3296
36	618916.1453
37	619366.5115
38	619700.8157
39	620459.7256
40	621278.5921
41	622424.8979
42	624094.2989
43	625668.1934
44	627229.8438
45	627799.2929
46	628379.7492
47	628787.2531
48	629078.3611
49	629355.7608
50	629787.2895
51	630165.5652
52	630699.3978
53	631034.7318
54	631246.7961
55	631506.9853
56	631751.4338
57	631991.7702
58	632579.4319
59	633214.6266
60	633639.3415
61	633930.3866
62	634231.6121
63	634652.682
64	635024.66
65	635702.9833
66	636311.8014
67	637316.3676
68	638377.0006
69	639195.7807
70	640241.2023
71	640929.4167
72	641669.0715
73	642729.6936
74	644591.0413
75	646432.6184
76	647780.3333
77	649067.4796
78	650321.0104
79	651540.0983
80	652239.4835
81	653231.6213
82	653798.7798
83	654979.4623
84	655986.2309
85	656582.2792
86	657199.6684
87	657629.4702
88	658083.2323
89	658725.9371
90	659397.2247
91	659875.7953
92	660514.9986
93	661085.5812
94	661672.8188
95	662246.5445
96	662774.4549


==> Data/14-ITAGHC-IC96.tex <==
Design_Horizon	IT_IC
1	203000
2	203000
3	203000
4	203000
5	203000
6	203000
7	203000
8	203000
9	203000
10	203000
11	203000
12	203000
13	203000
14	203000
15	203000
16	203000
17	203000
18	203000
19	203000
20	203000
21	203000
22	203000
23	203000
24	203000
25	203000
26	203000
27	203000
28	203000
29	203000
30	203000
31	203000
32	203000
33	203000
34	203000
35	203000
36	203000
37	203000
38	203000
39	203000
40	203000
41	203000
42	203000
43	203000
44	203000
45	203000
46	203000
47	203000
48	203000
49	203000
50	203000
51	203000
52	203000
53	203000
54	203000
55	203000
56	203000
57	203000
58	203000
59	203000
60	203000
61	203000
62	203000
63	203000
64	203000
65	203000
66	203000
67	203000
68	203000
69	203000
70	203000
71	203000
72	203000
73	203000
74	203000
75	203000
76	203000
77	203000
78	203000
79	203000
80	203000
81	203000
82	203000
83	203000
84	203000
85	203000
86	203000
87	203000
88	203000
89	203000
90	203000
91	203000
92	203000
93	203000
94	203000
95	203000
96	203000


==> Data/14-ITAGHC-OC96.tex <==
Design_Horizon	IT_OC
1	1532.073418
2	3016.983309
3	6391.868722
4	9024.005204
5	12859.09568
6	14213.80312
7	16462.17893
8	17974.02728
9	19035.64626
10	19845.42787
11	20897.27798
12	21370.43172
13	21814.068
14	23333.98223
15	25320.12208
16	27567.92867
17	29042.81721
18	29457.38416
19	30246.54224
20	31157.2682
21	31628.57727
22	32051.95599
23	32487.75336
24	32853.38805
25	33219.20992
26	33598.94263
27	33986.54507
28	34363.72013
29	34741.55051
30	35559.79858
31	36101.91232
32	36705.21369
33	37247.81597
34	37725.46421
35	38324.45777
36	39192.62522
37	40265.42283
38	41088.80922
39	43084.15755
40	45254.73019
41	48322.96101
42	52793.76918
43	56949.62426
44	61075.22986
45	62452.47942
46	63868.68392
47	64851.97051
48	65566.16752
49	66243.48439
50	67285.89592
51	68216.36368
52	69483.82978
53	70315.83548
54	70794.05455
55	71430.21143
56	72015.5437
57	72588.89342
58	74030.34711
59	75634.64581
60	76655.66737
61	77376.2253
62	78122.96996
63	79136.73625
64	80046.55544
65	81794.34375
66	83309.15727
67	85999.97756
68	88842.65422
69	91013.07675
70	93814.83121
71	95596.38149
72	97538.51349
73	100385.2526
74	105419.0293
75	110392.2917
76	113989.6441
77	117431.8488
78	120788.0502
79	124054.8073
80	125872.505
81	128534.6169
82	129904.3132
83	133070.7654
84	135772.8616
85	137273.8647
86	138858.9194
87	139897.4472
88	140984.2549
89	142664.2082
90	144391.861
91	145525.0527
92	147144.6466
93	148528.728
94	149970.7904
95	151365.8478
96	152596.7864


==> Data/14-ITAGHC-TC96.tex <==
Design_Horizon	IT_TC
1	204532.0734
2	206016.9833
3	209391.8687
4	212024.0052
5	215859.0957
6	217213.8031
7	219462.1789
8	220974.0273
9	222035.6463
10	222845.4279
11	223897.278
12	224370.4317
13	224814.068
14	226333.9822
15	228320.1221
16	230567.9287
17	232042.8172
18	232457.3842
19	233246.5422
20	234157.2682
21	234628.5773
22	235051.956
23	235487.7534
24	235853.3881
25	236219.2099
26	236598.9426
27	236986.5451
28	237363.7201
29	237741.5505
30	238559.7986
31	239101.9123
32	239705.2137
33	240247.816
34	240725.4642
35	241324.4578
36	242192.6252
37	243265.4228
38	244088.8092
39	246084.1576
40	248254.7302
41	251322.961
42	255793.7692
43	259949.6243
44	264075.2299
45	265452.4794
46	266868.6839
47	267851.9705
48	268566.1675
49	269243.4844
50	270285.8959
51	271216.3637
52	272483.8298
53	273315.8355
54	273794.0545
55	274430.2114
56	275015.5437
57	275588.8934
58	277030.3471
59	278634.6458
60	279655.6674
61	280376.2253
62	281122.97
63	282136.7362
64	283046.5554
65	284794.3437
66	286309.1573
67	288999.9776
68	291842.6542
69	294013.0768
70	296814.8312
71	298596.3815
72	300538.5135
73	303385.2526
74	308419.0293
75	313392.2917
76	316989.6441
77	320431.8488
78	323788.0502
79	327054.8073
80	328872.505
81	331534.6169
82	332904.3132
83	336070.7654
84	338772.8616
85	340273.8647
86	341858.9194
87	342897.4472
88	343984.2549
89	345664.2082
90	347391.861
91	348525.0527
92	350144.6466
93	351528.728
94	352970.7904
95	354365.8478
96	355596.7864


==> Data/15-ITAGNLHC-IC96.tex <==
Design_Horizon	IT_IC
1	602513.7
2	602513.7
3	602513.7
4	602513.7
5	602513.7
6	602513.7
7	602513.7
8	602513.7
9	602513.7
10	602513.7
11	602513.7
12	602513.7
13	602513.7
14	602513.7
15	602513.7
16	602513.7
17	602513.7
18	602513.7
19	602513.7
20	602513.7
21	602513.7
22	602513.7
23	602513.7
24	602513.7
25	602513.7
26	602513.7
27	602513.7
28	602513.7
29	602513.7
30	602513.7
31	602513.7
32	602513.7
33	602513.7
34	602513.7
35	602513.7
36	602513.7
37	602513.7
38	602513.7
39	602513.7
40	602513.7
41	602513.7
42	602513.7
43	602513.7
44	602513.7
45	602513.7
46	602513.7
47	602513.7
48	602513.7
49	602513.7
50	602513.7
51	602513.7
52	602513.7
53	602513.7
54	602513.7
55	602513.7
56	602513.7
57	602513.7
58	602513.7
59	602513.7
60	602513.7
61	602513.7
62	602513.7
63	602513.7
64	602513.7
65	602513.7
66	602513.7
67	602513.7
68	602513.7
69	602513.7
70	602513.7
71	602513.7
72	602513.7
73	602513.7
74	602513.7
75	602513.7
76	602513.7
77	602513.7
78	602513.7
79	602513.7
80	602513.7
81	602513.7
82	602513.7
83	602513.7
84	602513.7
85	602513.7
86	602513.7
87	602513.7
88	602513.7
89	602513.7
90	602513.7
91	602513.7
92	602513.7
93	602513.7
94	602513.7
95	602513.7
96	602513.7


==> Data/15-ITAGNLHC-OC96.tex <==
Design_Horizon	IT_OC
1	475.2778368
2	925.4370048
3	2075.647171
4	2976.24905
5	4468.515984
6	5016.637509
7	5814.088379
8	6374.466775
9	6771.224129
10	7081.914422
11	7475.547053
12	7689.127028
13	7896.792087
14	8460.373751
15	9193.621151
16	10001.00638
17	10574.23575
18	10790.70546
19	11172.55531
20	11524.54067
21	11740.99907
22	11962.70295
23	12140.19563
24	12333.80073
25	12511.29341
26	12688.78609
27	12878.78277
28	13066.52296
29	13244.01564
30	13637.84084
31	13815.33351
32	14096.79392
33	14274.2866
34	14493.28553
35	14873.64903
36	15431.43195
37	15989.49676
38	16187.76847
39	16920.7631
40	17697.10593
41	18801.43755
42	20188.83619
43	21576.23483
44	22951.98327
45	23352.62284
46	23910.87609
47	24262.86144
48	24784.01862
49	24961.5113
50	25313.3427
51	25537.84794
52	26238.81865
53	26590.80401
54	26807.9531
55	27223.8269
56	27581.45687
57	27758.94955
58	28322.53847
59	28929.64794
60	29270.39999
61	29452.99163
62	29987.22012
63	30243.41088
64	30578.6586
65	31234.08351
66	31793.10209
67	32708.54661
68	33668.00567
69	34445.50653
70	35392.88456
71	36062.35239
72	36782.35535
73	37739.7407
74	39404.96769
75	41054.09587
76	42258.27716
77	43408.15777
78	44529.57448
79	45657.02422
80	46342.10626
81	47241.6091
82	47639.30962
83	48701.29987
84	49612.35837
85	50182.7568
86	50883.72751
87	51495.91472
88	52059.90759
89	52590.07084
90	53186.84818
91	53538.83353
92	54061.15439
93	54612.64443
94	55175.9215
95	55729.47951
96	56092.17225


==> Data/15-ITAGNLHC-TC96.tex <==
Design_Horizon	IT_TC
1	602988.9778
2	603439.137
3	604589.3472
4	605489.949
5	606982.216
6	607530.3375
7	608327.7884
8	608888.1668
9	609284.9241
10	609595.6144
11	609989.2471
12	610202.827
13	610410.4921
14	610974.0738
15	611707.3212
16	612514.7064
17	613087.9357
18	613304.4055
19	613686.2553
20	614038.2407
21	614254.6991
22	614476.403
23	614653.8956
24	614847.5007
25	615024.9934
26	615202.4861
27	615392.4828
28	615580.223
29	615757.7156
30	616151.5408
31	616329.0335
32	616610.4939
33	616787.9866
34	617006.9855
35	617387.349
36	617945.1319
37	618503.1968
38	618701.4685
39	619434.4631
40	620210.8059
41	621315.1375
42	622702.5362
43	624089.9348
44	625465.6833
45	625866.3228
46	626424.5761
47	626776.5614
48	627297.7186
49	627475.2113
50	627827.0427
51	628051.5479
52	628752.5187
53	629104.504
54	629321.6531
55	629737.5269
56	630095.1569
57	630272.6496
58	630836.2385
59	631443.3479
60	631784.1
61	631966.6916
62	632500.9201
63	632757.1109
64	633092.3586
65	633747.7835
66	634306.8021
67	635222.2466
68	636181.7057
69	636959.2065
70	637906.5846
71	638576.0524
72	639296.0553
73	640253.4407
74	641918.6677
75	643567.7959
76	644771.9772
77	645921.8578
78	647043.2745
79	648170.7242
80	648855.8063
81	649755.3091
82	650153.0096
83	651214.9999
84	652126.0584
85	652696.4568
86	653397.4275
87	654009.6147
88	654573.6076
89	655103.7708
90	655700.5482
91	656052.5335
92	656574.8544
93	657126.3444
94	657689.6215
95	658243.1795
96	658605.8723

